Fully Automatic Trunk Packing with Free Placements

We present a new algorithm to compute the volume of a trunk according to the SAE J1100 standard. Our new algorithm uses state-of-the-art methods from computational geometry and from combinatorial optimization. It finds better solutions than previous approaches for small trunks.

==> csps.tex <==
\section{Computation of the Feasible Area}

A \emph{configuration space} of an object $R$ defines set of all
placements of $R$, with respect to a set of obstacles
$S$~\cite{bkos-cgaa-97}. The placement may consist of a position and
an orientation of $R$ in a $d$-dimensional work space. It decomposes
into the \emph{forbidden space}, the set of configurations in which
$R$ intersects with $S$, and the \emph{free space}, the set of
configurations in which $R$ does not intersect $S$. In the trunk
packing scenario $R$ is a suitcase, $S$ is the complement of the
trunk's interior, and the configuration space is a six-dimensional
space defining all positions and orientation of $R$ in the
three-dimensional space. We look at a variant of the problem where the
orienation is limited to the six axis-aligned orientations.

If $R$ has only one orientation, e.g., $R$ is a translation robot, the
forbidden space, can be computed as the Minkowski sum $-R\oplus S =
\{r+o:r\in -R, s \in S \}$, where $-R$ is the inverted point set of $R$.
The Minkowski sum is a very complex operation. It is usually computed
by decomposing the two objects into convex pieces, computing all
pairwise Minkowski sums of the convex pieces, and uniting the pairwise
sums. In the three-dimensional space, this operation has complexity
$O(n^6)$, where $n$ is the combined complexity of $R$ and $S$. Our
approach to solve the trunk packing problem is based on the Minkowski
sum. We compute the free space of a suitcase with respect to a trunk
as six complements of Minkowski sums, one for each orientation.

There are a few implementations of three-dimensional non-convex
Minkowski sums~\cite{vm-, h-}, but none that supports infinite point
sets. Also, the trunk models usually have holes, which denies the
possibility to treat them, i.e., the boundary plus either the outer
space or the inside of the trunk, as a solid. Instead, we compute the
Minkowski sum of the suitcase and the boundary of the trunk, which can
be expressed as the union of all Minkowski sums of the suitcase and a
facet of the trunk. If the holes in the surface are not big enough for
the suitcase to fit through, the resulting polyhedron $B$ decomposes
the three-dimensional space into three regions: $B$, the region $N$
outside of $B$, and a void $F$ enclosed by $B$. Obviously, $B$ is a
subset of both, the Minkowski sum of trunk and suitcase, and the
Minkowski sum of the (closure of the) complement of the trunk and the
suitcase. Also, it is clear that $B$ includes the extreme points of
both Minkowski sums. Thus, $F$ is exactly the set of points where we
can place the suitcase within the trunk.

To compute $F$, we use polyhedral surfaces~\cite{} and 3D Nef
polyhedra~\cite{} provided by {\cgal}~\cite{}. The use of
{\cgal} is motivated by the many tools provided by {\cgal}'s packages
that allow us to consider several approaches for computing the free
space, and by robustness issues. The union step in the Minkowski sum
often includes many degenerate situations. As we wil see in the next
section, we also need a decomposition of a non-convex polyhedron into
convex pieces, which also features lots of degeneracy problems.

With the {\cgal} packages, the Minkowski sum of a suitcase and the
boundary of a trunk is easy to compute. The surfaces of our trunks
only consist of triangles. Since both, the facets of the trunk and the
suitcase, are convex, their Minkowski sum can be computed as the
convex hull of the vector sums of their vertices~\cite{Latombe}. The
output sensitive and therefore asymptotically faster method using
Gaussian maps can also be found in {\cgal}, but is not faster for
these small instances. We then use the binary operation of Nef
polyhedra and the heuristics described in \cite{h--07} to efficiently
compute the union of the convex Minkowski sums. 

A 3D Nef polyhedron in {\cgal} is represented as a subdivision of the
three-dimensional space. Each cell of the subdivision has a
set-selection mark. These marks indicate which cells form the
polyhedron, and which cells represent the rest of the
three-dimensional spaces. With the union of the convex Minkowski sums,
we have obtained a polyhedron with three three-dimensional cells
separated by boundary parts, where one of the cells, the one that
represents the union, and the boundary are selected, and the two
others are unselected. We now select the cell that represents th outer
volume and call the simplification routine of the Nef polyhedron
class. By selecting the outer volume the boundary between the outer
volume and the union becomes redundant and is remove by the
simplification routine. The complement of what is left is the desired
configuration space. 

With this method, the computation of the free space of trunk {\large}
with a fixed orientation takes 36 minutes on our machine. The choice
of the suitcase and its orientation does not influence the running
time considerably. For big suitcases sometimes 35 minutes was enough,
for small suitcases, it could take 37 minutes. For the trunks {\tiny},
{\small}, and {\medium} the compution times are 103, 66, and XX
minutes.

Because the described method is not very fast, we tried several
heuristics to speed up the union, which takes most of the
time. Without the holes in the trunk surfaces we could easily be much
faster as follows: We first transform the outer region into a solid by
setting the selection mark. Then we unite several copies of this
solid, where each copy is translated such that it represent an extreme
point on the trunk. This results in a fairly good first approximation
of the forbidden space. Up to this point, the approximation is a
subset of the forbidden space and it is left to check and add those
convex Minkowski sums that do not lie completely within this
approximation. The number of united polyhedra is expected to drop
considerably by this method. 

The crucial point of making this method fast is to get a good first
approximation of the forbidden space. The better the approximation the
more unions we can prune. Unfortunately, we don't know of any method
to automatically remove holes and removing them manually is extremely
tedious. So, we cannot start with the solid outside the trunk
boundary. Instead we started with the solid outside the convex hull of
the trunk or outside the bounding box of the trunk. But this approach,
albeit effective, is not reliable. It worked nicely for all but one of
our input sets. The problematic trunk is the trunk of a cabriolet,
which includes, apart from the boundary of the trunk interior, many
additional details that extends far from the for us relevant
parts. For such a model, a first approximation obtained by the convex
hull and the bounding box are too large. Converting the regions
outside either of these surfaces into a solid and adding all convex
Minkowski sums might leave several regions one of which is the search
free space, but we cannot determine which.

Our most successful heuristic just starts uniting the convex sums
until they form a closed surface. Then we convert the intermedite
union together with the outer volume into a solid and
continue. Because the the facets of the trunk are not in random order,
but usually construct the trunk side by side, we quickly get a closed
surface if we use the convex sums of every $x$th facet. Choosing $x$
just big enough to get a closed surface, quickly yields a good
approximation. We find a good $x$ by starting with $x=256$ checking
for a closed surface. If we don't find a closed surface we half $x$
and repeat.

With this method we often had good results. Our most impressive
improvement was the computation of a free space in 279 seconds instead
of 3889 second. But the performance is not reliable---sometimes a
closed surface is not found quickly---and it can also yield the wrong
result. That happens when we get a closed surface within a cluster of
boxes. Unfortunately, we cannot tell whether a closed surface extents
around the search free space or not.

Summing up, we would be interested in a reliable method to close holes
in a surface.  Without this step there seems to be no reliable method
to speed up the union of the convex sums.


==> hsp.tex <==
\section{Simplification of the Feasible Area}

To make the feasible area efficiently usable for the LP-solver, we
need to describe it as a set of allowed and forbidden convex
regions. Also, we want the description not to be too big. Out input
format for the LP-solver describes the feasible area by it's convex
hull minus a set of convex obstacles. We obtain this format by
computing the difference of the feasible area's convex hull and the
area itself, and then decomposing the difference into convex pieces
with the decomposition method described in~\cite{h-emspe-07}, which
will become part of \cgal\ with the next release. The decomposition
method inserts additional facets into the interior of the
polyhedron. The Nef polyhedron class allows to use a visitor class to
access the boundary of each cell separately. Thereby, we extract the
plane equations that define the facets of the convex hull and the
obstacles.

For the LP-solver it is important to distinguish halfspaces that
separates an obstacle from the feasible area, an obstacle from the
space outside the convex hull, or an obstacle from another
obstacle. The first type of halfspaces are the most promising position
for the placement of a suitcase, because they represent the extreme
positions of the suitcase within the trunk. The two other cases,
represent placements outside the feasible area and should not be
considered. We therefore store two separate lists of halfspaces for
each obstacle, one with halfspaces that are legal placements and one
with halfspaces that define forbidden positions. 

The resulting data sets are too big to allow fast solutions by the
LP-solver. In our experiments, the description of the feasible area
according to our data format usually comprises several hundred
obstacles. In case of trunk $L$ and suitcase $H$ we had 4904
obstacles. The convex hull and a few of the obstacles are usually
described by a few hundred halfspaces, the rest of the obstacles by
around 6-40 facets. Our largest data set is described by a total of
72554 halfspaces. We therefore want to simplify the data sets, without
changing the represented point set too much. Most important, we don't
want the represented point set to contain any points outside the
feasible area.

Our simplification approach unites adjacent obstacles. Because such a
union is usually non-convex, we replace the obstacles by their
combined convex hull. The convex hulls of obstacles are surely bigger
than the union of the replaced obstacles and will therefore overlap
parts of the feasible area. More precisely, because of the structure
of the decomposition, it is unlikely that the convex hull of two
adjacent obstacles overlap a third obstacle, and surely it cannot
overlap the region outside the convex hull of the feasible area. Since
we want to shrink the represented point set as few as possible, we
need ways to measure the region. For this purpose we adapted the code
of Mirtich's volume integration method~\cite{m-facpm-96}, such that it
computes the volume of a cell of a Nef polyehdron. Now we replace two
obstacles by their combined convex hull, if this convex hull is either
not more than a certain percentage larger than their combined convex
hull, or not more than a fixed volume larger. The replacement process
is done iteratively as long as we find obstacle pairs that can be
joined according to the given percentage and the given fixed
volume. Note, that we maintain the volume of the union of each set of
joined obstacles. Thus, to test for replacement, we always compare the
volume of a convex hull of a set of obstacles, with the volume of
their union. To find candidate obstacle pairs, we just iterate in
random order over all facets separating two obstacles and check
whether they qualify to be replaced by their combined convex hull. If
they do, we replace them immediately.

